Benchmarking Cognitive Biases in Large Language Models as Evaluators

Large Language Models are cognitively biased judges. Large Language Models (LLMs) have recently been shown to be effective as automatic evaluators with simple prompting and in-context learning. In this work, we assemble 15 LLMs of four different size ranges and evaluate their output responses by preference ranking from the other LLMs as evaluators, such as System Star is better than System Square. We then evaluate the quality of ranking outputs introducing the Cognitive Bias Benchmark for LLMs as Evaluators (CoBBLEr), a benchmark to measure six different cognitive biases in LLM evaluation outputs, such as the Egocentric bias where a model prefers to rank its own outputs highly in evaluation. We find that LLMs are biased text quality evaluators, exhibiting strong indications on our bias benchmark (average of 40% of comparisons across all models) within each of their evaluations that question their robustness as evaluators. Furthermore, we examine the correlation between human and machine preferences and calculate the average Rank-Biased Overlap (RBO) score to be 49.6%, indicating that machine preferences are misaligned with humans. According to our findings, LLMs may still be unable to be utilized for automatic annotation aligned with human preferences. Our project page is at: https://minnesotanlp.github.io/cobbler.

==> tables/human_bias.tex <==
% \begin{table*}[t!]
% \footnotesize
% \begin{tabularx}{0.6\linewidth}{@{}p{1.5cm}P{1.8cm}P{1.8cm}P{1.8cm}P{0.8cm}@{}}\toprule
% & \multicolumn{2}{c}{\scriptsize{\textsc{Order}}} & \scriptsize{\textsc{Salience}} & \scriptsize{\textsc{Bandwag.}}  & \scriptsize{\textsc{Attent.}} \\
% % \cmidrule{4-5} \cmidrule{7-8}
%  & \scriptsize{First} & \scriptsize{Last} & &  &  &  & & & & \\
% \midrule
% % Section (a) 
% \textsc{Human} & 0.20 & 0.18 & 0.52 & 0.47 & 0.35 \\
% \midrule
% % Section (b)
% \textsc{GPT-4} & 0.17 & 0.06 & 0.56 & 0.0 & 0.0 \\
% \bottomrule
% \end{tabularx}
% \caption{the proportion of pairs identified as biased responses across all human annotators for \textsc{Order}, \textsc{Salience}, \textsc{Bandwagon}, and \textsc{Attetional} biases. Similarly, a higher score indicates more biased performance.}
% \label{results:human-bias}
% \end{table*}

\begin{table}[t!]
\centering
\begin{tabularx}{0.65\linewidth}
{@{}p{1.5cm}P{3cm}P{3cm}P{3cm}P{3cm}@{}}
\toprule
& \multicolumn{2}{x}{\scriptsize{\textsc{Order}}} & \scriptsize{\textsc{Salience}} & \scriptsize{\textsc{Bandwagon}}  & \scriptsize{\textsc{Attentional}} \\
% \cmidrule{4-5} \cmidrule{7-8}
 & \scriptsize{First} & \scriptsize{Last} & &  &  &  &  
\\
\midrule
% Section (a) 
\textsc{Human} & 0.20 & 0.18 & 0.52 & 0.47 & 0.35 \\
\midrule
% Section (b)
\textsc{Vicuna} & 0.32 & 0.17 & 0.53 & 0.81 & 0.78 \\
\bottomrule
    \end{tabularx}
% }
\caption{The proportion of biased responses across all human annotators for \textsc{Order Bias}, \textsc{Salience Bias}, \textsc{Bandwagon Effect}, and \textsc{Attentional Bias}, as a comparison with \textsc{Vicuna}. Similarly with Table \ref{results:main}, a higher score indicates more biased performance.}
\label{results:human-bias}
\end{table}

==> tables/qualitative_preference.tex <==
% \newcommand{\tinysc}[1]{\tiny{\textsc{#1}}}

% \begin{table}[t!]
%   \centering
%   \scriptsize
%   \begin{tabularx}{\linewidth}{*{11}{>{\arraybackslash}X}}
%     \toprule
%     \multicolumn{5}{c}{\parbox{5.4cm}{\texttt{Instruction: Did people in Korea under Japanese Rule watch a lot of Iron Chef?}}} & 
%     \multicolumn{5}{c}{\parbox{5.7cm}{\texttt{Instruction: Why classical music still sounds good today (after four hundred years), but lots of music from even ten years ago sounds lame?}}} \\
%     % \multicolumn{4}{c}{\parbox{4.0cm}{Instruction: Did Brazilian jiu-jitsu Gracie founders have at least a baker's dozen of kids between them?}} \\
%     \cmidrule(lr){1-5}  \cmidrule(lr){6-10} 
%     % \cmidrule(lr){9-12}
%     \scriptsize{\textsc{GPT4}} & \scriptsize{\textsc{Cohere}} & \scriptsize{\textsc{Vicuna}} &\scriptsize{\textsc{MPT}} & \scriptsize{\textsc{Human}}
%     & \scriptsize{\textsc{GPT4}} & \scriptsize{\textsc{Cohere}} & \scriptsize{\textsc{Vicuna}} & \scriptsize{\textsc{MPT}} & \scriptsize{\textsc{Human}} \\
%     % & \tiny{\textsc{GPT4}} & \tiny{\textsc{Cohere}} & \tiny{\textsc{MPT}} & \tiny{\textsc{Human}} \\
%     \midrule
%     \cellcolor{yellow!25}\tiny{\textsc{GPT4}} & \tinysc{Baize} & \cellcolor{yellow!25}\tinysc{GPT4}& \tinysc{Baize} & \tinysc{GPT4}  %%
%     & \tinysc{GPT4} & \tinysc{Instruct} &  \tinysc{Vicuna} & \cellcolor{yellow!25}\tinysc{Baize} &  \tinysc{Baize} \\
    
%     \tiny{\textsc{WizardLM}} & \tinysc{GPT4} & \tinysc{Cohere}& \tinysc{WizardLM} & \tinysc{Vicuna} %%
%     & \tinysc{ChatGPT} & \cellcolor{yellow!25}\tinysc{Vicuna} & \tinysc{WizardLM} & \tinysc{WizardLM} & \tinysc{Vicuna} \\
    
%     \tiny{\textsc{ChatGPT}} & \tinysc{WizardLM} & \tinysc{Baize} & \tinysc{Alpaca} & \tinysc{Cohere} %%
%     & \tinysc{Falcon} & \tinysc{WizardLM} & \tinysc{Baize} & \tinysc{ChatGPT} & \tinysc{Koala}\\
    
%     \tiny{\textsc{Baize}} & \tinysc{Cohere} & \tinysc{Instruct} & \tinysc{MPT} & \tinysc{ChatGPT} %%
%     & \tinysc{Baize} &  \tinysc{Alpaca} & \tinysc{Koala} & \tinysc{Vicuna} & \tinysc{Instruct} \\
    
%     \tiny{\textsc{Cohere}} & \tinysc{Alpaca} & \tinysc{Dolly} & \tinysc{GPT4} & \tinysc{WizardLM} %%
%     & \tinysc{OpenAssist} & \tinysc{Koala} & \cellcolor{yellow!25}\tinysc{ChatGPT} & \tinysc{Instruct} & \tinysc{ChatGPT}\\ 
%     \bottomrule
%   \end{tabularx}
%   \caption{Two examples of the (top-4) rankings for each LM-as-evaluator of the four model sizes compared to the average human rankings. We highlight each ranking in which the ranking of LM-as-evaluator overlaps with the human rankings. Full ranking data can be viewed on our project page.}
%   \vspace{-0.5cm}
%   \label{tab:qualitative}
% \end{table}

\newcommand{\tinysc}[1]{\tiny{\textsc{#1}}}

\begin{table}[t!]
  \centering
  \scriptsize
  \begin{tabularx}{\linewidth}{*{11}{>{\arraybackslash}X}}
    \toprule
    \multicolumn{5}{c}{\parbox{5.4cm}{\texttt{Instruction: Did people in Korea under Japanese Rule watch a lot of Iron Chef?}}} & 
    \multicolumn{5}{c}{\parbox{5.7cm}{\texttt{Instruction: Why classical music still sounds good today (after four hundred years), but lots of music from even ten years ago sounds lame?}}} \\
    % \multicolumn{4}{c}{\parbox{4.0cm}{Instruction: Did Brazilian jiu-jitsu Gracie founders have at least a baker's dozen of kids between them?}} \\
    \cmidrule(lr){1-5}  \cmidrule(lr){6-10} 
    % \cmidrule(lr){9-12}
    \scriptsize{\textsc{GPT4}} & \scriptsize{\textsc{Cohere}} & \scriptsize{\textsc{Vicuna}} &\scriptsize{\textsc{MPT}} & \scriptsize{\textsc{Human}}
    & \scriptsize{\textsc{GPT4}} & \scriptsize{\textsc{Cohere}} & \scriptsize{\textsc{Vicuna}} & \scriptsize{\textsc{MPT}} & \scriptsize{\textsc{Human}} \\
    % & \tiny{\textsc{GPT4}} & \tiny{\textsc{Cohere}} & \tiny{\textsc{MPT}} & \tiny{\textsc{Human}} \\
    \midrule
    \cellcolor{yellow!25}\tiny{\textsc{GPT4}} & \tinysc{Baize} & \cellcolor{yellow!25}\tinysc{GPT4}& \tinysc{Baize} & \tinysc{GPT4}  %%
    & \tinysc{GPT4} & \tinysc{Instruct} &  \tinysc{Vicuna} & \cellcolor{yellow!25}\tinysc{Baize} &  \tinysc{Baize} \\
    
    \tiny{\textsc{WizardLM}} & \tinysc{GPT4} & \tinysc{Cohere}& \tinysc{WizardLM} & \tinysc{Vicuna} %%
    & \tinysc{ChatGPT} & \cellcolor{yellow!25}\tinysc{Vicuna} & \tinysc{WizardLM} & \tinysc{WizardLM} & \tinysc{Vicuna} \\
    
    \tiny{\textsc{ChatGPT}} & \tinysc{WizardLM} & \tinysc{Baize} & \tinysc{Alpaca} & \tinysc{Cohere} %%
    & \tinysc{Falcon} & \tinysc{WizardLM} & \tinysc{Baize} & \tinysc{ChatGPT} & \tinysc{Koala}\\
    
    \tiny{\textsc{Baize}} & \tinysc{Cohere} & \tinysc{Instruct} & \tinysc{MPT} & \tinysc{ChatGPT} %%
    & \tinysc{Baize} &  \tinysc{Alpaca} & \tinysc{Koala} & \tinysc{Vicuna} & \tinysc{Instruct} \\
    
    % \tiny{\textsc{Cohere}} & \tinysc{Alpaca} & \tinysc{Dolly} & \tinysc{GPT4} & \tinysc{WizardLM} %%
    % & \tinysc{OpenAssist} & \tinysc{Koala} & \cellcolor{yellow!25}\tinysc{ChatGPT} & \tinysc{Instruct} & \tinysc{ChatGPT}\\ 
    \bottomrule
  \end{tabularx}
  \caption{Two examples of the (top-4) rankings for each LM-as-evaluator of the four model sizes compared to the average human rankings. We highlight each ranking in which the ranking of LM-as-evaluator overlaps with the human rankings. Full ranking data can be viewed on our project page.}
  \vspace{-0.5cm}
  \label{tab:qualitative}
\end{table}


==> tables/validity_results.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{l|c|p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}}\toprule
\textbf{Model} & \textbf{Avg.} & Ord. & Comp. & Band. & Atte. \\
\midrule
\textsc{GPT4} & 0.987 & 0.989 & 0.978 & 0.991 & 0.998 \\
\textsc{ChatGPT} & 0.997 & 0.997 & 0.996 & 0.999 & 0.998 \\
\textsc{InstructGPT} & 0.998 & 0.999 & 0.999 & 1.000 & 0.997 \\
\midrule
\textsc{LLaMA} &  0.144 & 0.226 & 0.169 & 0.035 & 0.589\\
\textsc{Cohere} &  0.982 & 0.940 & 0.995 & 0.820 & 0.998 \\
\textsc{Falcon} &  0.726 & 0.721 & 0.461 & 0.993 & 0.986 \\
\midrule
\textsc{Alpaca} & 0.846 & 0.782 & 0.828 & 0.979 & 0.877 \\
\textsc{Vicuna} & 0.866 & 0.901 & 0.719 & 0.974 & 0.901\\
\textsc{OpenAssist} & 0.600 & 0.800 & 0.322 & 0.953 & 0.945 \\
\textsc{DollyV2} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\midrule
\textsc{Baize} &  0.964 & 0.986 & 0.875 & 0.997 & 0.995 \\
\textsc{Koala} &  0.258 & 0.295 & 0.185 & 0.230 & 0.302  \\
\textsc{WizardLM} & 0.937 & 0.953 & 0.830 & 0.997 & 0.967\\
\textsc{MPT} & 0.779 & 0.820 & 0.724 & 0.845 & 0.322 \\
\textsc{RedPajama} & 0.522 & 0.526 & 0.265 & 0.725 & 0.656\\
\bottomrule
\end{tabular}
\caption{Model performance for generating sensible evaluations. A higher percentage indicates a higher rate in which each \textit{eval-gen} properly chose a winner for each pairwise comparison.}
\label{results:validity}
\end{table}
